Royal Reveals: LiDAR Mapping of Kronborg Castle, Echoes of Hamlet's Halls

This paper presents a large scale dataset from a meticulous 360-degree LiDAR (Light Detection and Ranging) scan conducted on Kronborg Castle, a renowned Renaissance fortress located in Elsinore (Helsing{\o}r), Denmark, famously associated with Shakespeare's "Hamlet." Utilising a vertical mounted, gimbal stabilised, 16 channel, 360-degree Velodyne VLP-16 LiDAR scanner, paired with an Intel RealSense L515 depth camera. This research offers an unparalleled digital representation of the castle's intricate architectural details and structural nuances, enabling fellow researchers to conduct experiments utilising the data for SLAM (Simultaneous Localisation and Mapping) as well as floorplan generation.

==> Figures/full_pointcloud.tex <==
                \begin{figure}
            \centering
            \includegraphics[width=0.50\linewidth]{Figures/Pointcloud_images/All_Layers_Top.png}
            \caption{Scanning aparatus}
            \label{fig:enter-label}
        \end{figure}

==> Figures/gimbal.tex <==
                \begin{figure}
            \centering
            \includegraphics[width=0.50\linewidth]{Figures/Gimbal.JPEG}
            \caption{Scanning aparatus}
            \label{fig:enter-label}
        \end{figure}

==> Tables/Floor_Plans.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{|>{\centering\arraybackslash}m{4cm}|c|}
        \hline
        \textbf{Floor} & \textbf{Floor Plan} \\
        \hline
        Basement & \includegraphics[width=0.25\textwidth]{Figures/floor_plans/basement.jpg} \\
        \hline
        Ground Floor & \includegraphics[width=0.25\textwidth]{Figures/floor_plans/ground_floor.jpg} \\
        \hline
        First Floor & \includegraphics[width=0.25\textwidth]{Figures/floor_plans/first_floor.jpg} \\
        \hline
        Second Floor & \includegraphics[width=0.25\textwidth]{Figures/floor_plans/second_floor.jpg} \\
        \hline
        Third Floor (Attic) & \includegraphics[width=0.25\textwidth]{Figures/floor_plans/attic.jpg} \\
        \hline
    \end{tabular}
    \caption{Kronborg Castle: Floor Plan}
    \label{tab:floor_plans}
\end{table}
